Toward Practical Entity Alignment Method Design: Insights from New Highly Heterogeneous Knowledge Graph Datasets

The flourishing of knowledge graph applications has driven the need for entity alignment (EA) across KGs. However, the heterogeneity of practical KGs, characterized by differing scales, structures, and limited overlapping entities, greatly surpasses that of existing EA datasets. This discrepancy highlights an oversimplified heterogeneity in current EA datasets, which obstructs a full understanding of the advancements achieved by recent EA methods. In this paper, we study the performance of EA methods in practical settings, specifically focusing on the alignment of highly heterogeneous KGs (HHKGs). Firstly, we address the oversimplified heterogeneity settings of current datasets and propose two new HHKG datasets that closely mimic practical EA scenarios. Then, based on these datasets, we conduct extensive experiments to evaluate previous representative EA methods. Our findings reveal that, in aligning HHKGs, valuable structure information can hardly be exploited through message-passing and aggregation mechanisms. This phenomenon leads to inferior performance of existing EA methods, especially those based on GNNs. These findings shed light on the potential problems associated with the conventional application of GNN-based methods as a panacea for all EA datasets. Consequently, in light of these observations and to elucidate what EA methodology is genuinely beneficial in practical scenarios, we undertake an in-depth analysis by implementing a simple but effective approach: Simple-HHEA. This method adaptly integrates entity name, structure, and temporal information to navigate the challenges posed by HHKGs. Our experiment results conclude that the key to the future EA model design in practice lies in their adaptability and efficiency to varying information quality conditions, as well as their capability to capture patterns across HHKGs.

==> sections/Preliminary_and_Related_Works.tex <==
% In this section, we introduce related embedding-based EA methods from three perspectives: Translation-based methods, GNN-based methods, and Other methods.

% \subsection{Knowledge Graph (KG)}
% Knowledge graph (KG) $\mathcal{KG} = (\mathcal{E}, \mathcal{R}, \mathcal{Q})$ stores the real-world knowledge in the form of facts $\mathcal{Q}$, given a set of entities $\mathcal{E}$ and relations $\mathcal{R}$, the $ {(e_{head}, r, e_{tail})} \in \mathcal{E}\times \mathcal{R}$ denotes the set of facts $\mathcal{Q}$, where $e_{head}, e_{tail} \in \mathcal{E}$ respectively denote the head entity and tail entity, $r \in \mathcal{R}$ denotes the relation.
% Besides, we also model the temporal information in KGs, given timestamps $\mathcal{T}$, we denote $t \in \mathcal{T}$ as the temporal information of the facts, and each fact is represented in the form of ${(e_{head}, r, e_{tail},t)}$.


% Based on the basic concept of the KGs, we proposed a concept called highly heterogeneous knowledge graphs (HHKGs). Specifically, it is a relative concept, and indicates that the source KG and the target KG are far different from each other in scale, structure and overlapping ratios.

% To better illustrate the proposed concept, we also give a detailed statistics and analysis of our proposed highly heterogeneous KG datasets.
%这里给出知识图谱的基本介绍，并且通过对比引入Highly Heterogeneous Knowledge Graphs (HHKGs) 的概念。
%我在想这里是否还需要给出一个例子

% \subsection{Entity Alignment}
% %这里给出EA的任务定义，以及在后面给出分析为什么HHKG上EA更难，这里我在定义的层面强调出HHKG
% % Given two KGs $\mathcal{KG}_1 = (\mathcal{E}_1, \mathcal{R}_1, \mathcal{Q}_1)$ and $\mathcal{KG}_2 = (\mathcal{E}_2, \mathcal{R}_2, \mathcal{Q}_2)$, entity alignment (EA) aims to obtain the identical entity set $\mathcal{S} = \{(e_i, e_j)\|e_i\in \mathcal{E}_1, e_j \in \mathcal{E}_2\}$, where $e_i$ and $e_j$ represent the same real-world entity.

% % There has been research on various tasks similar to entity alignment.
% % \textit{Entity matching}~\cite{wang2011entity} is a counterpart problem of EA, which aims to align entities from two different relational databases (rather than KGs).
% % \textit{Entity resolution}~\cite{getoor2012entity} and \textit{entity linking}~\cite{shen2014entity} aim to match entities that are extracted from texts to corresponding entities in a KG.

% % In this paper, we research the problem of EA on highly heterogeneous KGs, which is extremely challenging because the correlation between HHKGs is not easy to leverage.
% %这里从定义层面把HHEA提出来
% %这里可以简要提出entity matching，entity resolution

% Entity alignment (EA) plays a crucial role in the field of knowledge graph research. Given two KGs, $\mathcal{KG}_1 = (\mathcal{E}_1, \mathcal{R}_1, \mathcal{Q}_1)$ and $\mathcal{KG}_2 = (\mathcal{E}_2, \mathcal{R}_2, \mathcal{Q}_2)$, the goal of EA is to determine the identical entity set $\mathcal{S} = {(e_i, e_j)|e_i\in \mathcal{E}_1, e_j \in \mathcal{E}_2}$. In this set, each pair $(e_i, e_j)$ represents the same real-world entity but exists in different KGs.

% % In addition to EA, there is a related task called \textit{Entity matching}~\cite{wang2011entity}. It is similar to EA in essence but focuses on aligning entities from two different relational databases instead of KGs. This task is primarily concerned with the alignment of structured data in databases.

% % Another two pertinent tasks are \textit{Entity resolution}\cite{getoor2012entity} and \textit{Entity linking}\cite{shen2014entity}.
% % \textit{Entity resolution} aims to identify and match entities that are referenced multiple times within a single data source or across different data sources.
% % \textit{Entity linking} aims to connect entities extracted from unstructured text data with the corresponding entities in a KG. They plays a pivotal role in enriching KGs with new knowledge and enhancing KGs' usability in various applications.

% The scope of this paper is primarily concerned with the problem of EA, particularly when applied to HHKGs. This is a challenging task due to the high degree of heterogeneity and complexity found in HHKGs. The structure and semantic correlations among entities in HHKGs are often intricate and convoluted, making it difficult to utilize these correlations effectively for EA. Therefore, our goal is to explore and develop methods that can handle these challenges efficiently and accurately, thereby pushing the boundaries of EA research in the context of HHKGs.

\textbf{Translation-based Entity Alignment.}
Translation-based EA approaches~\cite{chen2017multilingual, sun2017cross, sun2018bootstrapping, zhu2017iterative} are inspired by the TransE mechanism~\cite{bordes2013translating}, focusing on knowledge triplets $(u, r, v)$. Their scoring functions assess the triplet's validity to optimize knowledge representation. MTransE~\cite{chen2017multilingual} uses a translation mechanism for entity and relation embedding, leveraging pre-aligned entities for vector space transformation. Both AlignE~\cite{sun2018bootstrapping} and BootEA~\cite{sun2018bootstrapping} adjust aligned entities within triples to harmonize KG embeddings, with BootEA incorporating bootstrapping to address limited training data.

\textbf{GNN-based Entity Alignment.}
GNNs, designed to represent graph-structured data using deep learning, have become pivotal in EA tasks~\cite{wang2018cross, MuGNN, RNM, RREA, MRAEA}. Foundational models like GCN~\cite{kipf2016semi} and GAT~\cite{velivckovic2017graph} create entity embeddings by aggregating neighboring entity data, with GAT emphasizing crucial neighbors through attention. GCN-Align~\cite{wang2018cross} exemplifies GNN-based EA methods, utilizing GCN for unified semantic space entity embedding. Enhancements like RDGCN~\cite{wu2019relation} and Dual-AMN~\cite{mao2021boosting} introduced features to optimize neighbor similarity modeling. Recent methodologies, e.g., TEA-GNN~\cite{xu2021time}, TREA~\cite{xu2022time}, and STEA~\cite{STEA}, have integrated temporal data, underscoring its significance in EA tasks. A fundamental assumption of these methods is the similarity in neighborhood structures across entities, yet its universality remains unexplored.

\textbf{Others.}
Certain EA approaches transcend the above bounds. PARIS~\cite{suchanek2011paris} aligns entities in KGs using iterative probabilistic techniques, considering entity names and relations. Fualign~\cite{wang2023fualign} unifies two KGs based on trained entity pairs, learning a collective representation. BERT-INT~\cite{tang2020bert} addresses KG heterogeneity by solely leveraging side information, outperforming existing datasets. However, its exploration of KG heterogeneity remains limited to conventional datasets, not capturing the nuances of practical HHKGs.

==> sections/ccsxml.tex <==
\begin{CCSXML}
<ccs2012>
<concept>
<concept>
<concept_id>10010147.10010341.10010346.10010348</concept_id>
<concept_desc>Computing methodologies~Network science</concept_desc>
<concept_significance>500</concept_significance>
</concept>
<concept>
<concept_id>10010147.10010257.10010293.10010294</concept_id>
<concept_desc>Computing methodologies~Neural networks</concept_desc>
<concept_significance>500</concept_significance>
</concept>
</ccs2012>
\end{CCSXML}

\ccsdesc[500]{Information systems~Information integration}
% \ccsdesc[500]{Computing methodologies~Network science}
% \ccsdesc[500]{Computing methodologies~Neural networks}
